Adaptive Deep Learning for Entity Resolution by Risk Analysis

The state-of-the-art performance on entity resolution (ER) has been achieved by deep learning. However, deep models are usually trained on large quantities of accurately labeled training data, and can not be easily tuned towards a target workload. Unfortunately, in real scenarios, there may not be sufficient labeled training data, and even worse, their distribution is usually more or less different from the target workload even when they come from the same domain. To alleviate the said limitations, this paper proposes a novel risk-based approach to tune a deep model towards a target workload by its particular characteristics. Built on the recent advances on risk analysis for ER, the proposed approach first trains a deep model on labeled training data, and then fine-tunes it by minimizing its estimated misprediction risk on unlabeled target data. Our theoretical analysis shows that risk-based adaptive training can correct the label status of a mispredicted instance with a fairly good chance. We have also empirically validated the efficacy of the proposed approach on real benchmark data by a comparative study. Our extensive experiments show that it can considerably improve the performance of deep models. Furthermore, in the scenario of distribution misalignment, it can similarly outperform the state-of-the-art alternative of transfer learning by considerable margins. Using ER as a test case, we demonstrate that risk-based adaptive training is a promising approach potentially applicable to various challenging classification tasks.

==> 9-moreexperiments.tex <==

\section{Experimental Settings and More Evaluation}

\subsection{Datasets}
\label{appendix:datasets}

\begin{table}[ht]
	\caption{The statistics of datasets.}
	\label{tab:datasets}
	\begin{center}
		\begin{small}
			\begin{sc}
				\begin{tabular}{lccc}
					\toprule
					Dataset & Size & \# Matches & \# Attributes \\
					\midrule
					DS & 28,707 & 5,347 & 4 \\
					DA & 12,363 & 2,220 & 4 \\
					Cora & 12,674 & 3,268 & 12 \\
					AB & 9,575 & 1,028 & 3 \\
					IA & 539 & 132 & 8 \\
					SG & 19,633 & 6,108 & 7 \\
					\bottomrule
				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
\end{table}

In the \emph{Music} domain, besides the SG dataset, we also used the Itunes-Amazon dataset (denoted by IA) provided by \citet{githubdeepmatcher}. The size of IA is relatively small, containing only 539 pairs. As usual, on all the datasets, we used the blocking technique to filter the pairs deemed unlikely to match. The datasets of DS, DA, AB and IA have been made online available at \citet{githubdeepmatcher}. On both Cora and SG, we first filtered the pairs and then randomly selected a proportion of the resulting candidates to generate the workloads. The statistics of the test datasets are given in Table~\ref{tab:datasets}.


\subsection{Evaluation: Same Source}

\begin{figure*}[ht]
	\begin{center}
		\subfigure[DS.]
		{\includegraphics[width=0.31\linewidth]{figures/DS.pdf}}
		\subfigure[Cora.]
		{\includegraphics[width=0.31\linewidth]{figures/cora.pdf}}
		\subfigure[IA.]
		{\includegraphics[width=0.31\linewidth]{figures/IA.pdf}}
		\caption{Comparative evaluation: the same-source scenario.}
		\label{fig:exp-comparison}
	\end{center}
\end{figure*}

The additional evaluation results on the DS, Cora and IA datasets are presented in the Figure~\ref{fig:exp-comparison}. Similarly, it can be observed that \emph{Risk} achieves considerably better performance than \emph{Tradition} when training data are insufficient. Due to the small size of IA, the comparative results on IA have higher randomness compared with other datasets.


\subsection{Robustness w.r.t Size of Validation Data}


\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=0.33\columnwidth]{figures/sensitivity_SG.pdf}
		\caption{Robustness evaluation on SG dataset.}
		\label{fig:sg-sensitivity}
	\end{center}
\end{figure}

The evaluation results of robustness w.r.t size of validation data on SG dataset are presented in the Figure~\ref{fig:sg-sensitivity}. The evaluation for SG is also based on the setting that 10\% of the split set of training data is used. Similarly, it can be observed that \emph{Risk} is able to improve classifier performance by considerable margins with a very small set of validation data.

